Fine-Tuning BERTs for Definition Extraction from Mathematical Text

In this paper, we fine-tuned three pre-trained BERT models on the task of "definition extraction" from mathematical English written in LaTeX. This is presented as a binary classification problem, where either a sentence contains a definition of a mathematical term or it does not. We used two original data sets, "Chicago" and "TAC," to fine-tune and test these models. We also tested on WFMALL, a dataset presented by Vanetik and Litvak in 2021 and compared the performance of our models to theirs. We found that a high-performance Sentence-BERT transformer model performed best based on overall accuracy, recall, and precision metrics, achieving comparable results to the earlier models with less computational effort.

==> name.tex <==
\section{Discussion}
\subsection{Evaluation of results}
Overall we were surprised that in almost every metric SBERT outperformed both MathBERT models on all three datasets. Even more surprising was the relatively poorer performance of the enhanced vocabulary MathBERT2 model across all datasets. In general, our fine-tuned SBERT model was able to perform best on the Chicago dataset, which was the set with the highest density of definitions. Its performance on the combined dataset demonstrates that it was able to generalize to a dataset with a lower density of definition with minimal losses in performance. 

On the other hand, all three models showed low recall on the TAC dataset, which is most likely a result of low definition density. Additionally, the pre-training tasks for both MathBERT models implemented symbolic representations of mathematical text, rather than \LaTeX{} strings which could be an indication that they could be better leveraged if fine-tuned on pdf-scraped strings, rather than \LaTeX{} sentences. Regardless, the reduced performance of domain-specific transformer models on \LaTeX{} strings suggests that the use of models optimized for semantic and syntactic similarity is likely more appropriate for the task of definition classification. 



\subsection{Comparison of datasets}

There are a few indications that the labeled datasets we created were not optimal for fine-tuning models that could generalize to larger corpora of mathematical text. 

The TAC dataset had a low density of positive definition examples (7.53\% of the sentences were annotated as definitional), resulting in very low recall. During training, all three models developed a strategy of rejecting all examples of positive definitions in the training set, but were able to slightly recover in later epochs. Recall remains low, which directs us to expand on the fine-tuning process by implementing more balanced dataset for future work. When the pre-trained models were instead fine-tuned using the combined dataset the recall improved significantly, suggesting that by improving the definition density the performance of all models could be improved. 

To ensure that the improved performance was not due to the models optimizing only on the Chicago dataset elements while failing to generalize to the TAC dataset elements, we examined the isolated performance on subsets of elements from only one of the two datasets. These sentence label pairs had been isolated for validation and were not involved in the fine-tuning of the combined model. Tables \ref{table4} and \ref{table5} relate the performance of the SBERT model trained on the combined dataset on isolated subsets of the validation set for each dataset. We used the SBERT model to perform the confirmation because this model was best able to generalize across different datasets in the experiment. The Chicago validation subset consisted of 50 examples, whereas the TAC validation subset consisted of 100 examples due to its much larger size. 

\begin{table}[htbp]
    \centering
    \caption{Chicago Validation}
    \label{table4}
    \footnotesize
   \begin{tabularx}{\columnwidth}{|X|X|X|X|X|X|}
        \hline
         & Prec. & Rec. & F1 & Support & Acc.\\
        \hline
        $\neg$Def. & 0.96 & 0.89 & 0.93 & 28 &\\
        \hline
         Def. & 0.88 & 0.95 & 0.91 & 22 & 0.92 \\
    
        \hline
    \end{tabularx}
    \label{tab:Chicago_Validation}

   \caption{TAC Validation}
   \label{table5}
   \footnotesize
   \begin{tabularx}{\columnwidth}{|X|X|X|X|X|X|}
        \hline
         & Prec. & Rec. & F1 & Support & Acc.\\
        \hline
        $\neg$Def. & 0.99 & 1.00 & 0.99 & 98 &\\
        \hline
         Def. & 1.00 & 0.50 & 0.67 & 2 & 0.99 \\
    
        \hline
    \end{tabularx}
    \label{tab:TAC_Validation}
    
\end{table}

We confirmed our suspicion that the low density of TAC works against the recall of the model for positive examples, but we note that recall has improved even for the TAC subset over the results obtained from the models that were fine-tuned only on TAC. By combining datasets, performance also improves on the data for which there were few positive examples, leading us to conclude that generalization does occur.  The model fine-tuned on the combined dataset is capable of generalizing to some degree and we suspect that its generalization could be improved with a larger selection of training data. A clear area of improvement would be to ensure that the fine-tuning dataset has a sufficient number of positive examples. However, finding such datasets may be a persistent issue since mathematical definitions will usually make up a minority of sentences in any given mathematical corpus.  
